Ca substituion instead of Sr in La$_{0.58}$Sr$_{0.4}$Co$_{0.2}$Fe$_{0.8}$O$_{3-\delta}$ as a cathode electrode for IT-SOFCs

La$_{0.58}$Ca$_{0.4}$Co$_{0.2}$Fe$_{0.8}$O$_{3-\delta}$ (L58CCF) was synthesized and evaluated as a cathode electrode for intermediate temperature solid oxide fuel cells (IT-SOFC) based on the Y$_2$O$_3$-stabilized ZrO$_2$ (YSZ) electrolyte. The effect of sintering temperature on the L58CCF performance was investigated. The best Area specific resistances (ASRs) for the L58CCF sintered at 950 $^{\circ}$C were 1.218, 0.447, 0.228, 0.156, 0.099 $\Omega.cm^{2}$ at 600, 650, 700, 750, 800 $^{\circ}$C, respectively.

==> chapter3-1.tex <==
\bibliographystyle{elsarticle-num}



\section{supplementary}\label{Int}
Fig. 12 shows impurity percentage of L58CCF-1000, during heating and cooling in the temperature range 25-1200 °C.

\begin{figure}[!ht]
	\begin{center}
		\includegraphics[width=8cm,angle=0]{fig12}
		\vspace*{-0.4cm}
		\caption{ Impurity percentage for L58CCF-1000 tested in air from 25 to 1200 °C with consecutive heating/ cooling cycles.  
			\label{fig12}}
	\end{center}
\end{figure}

In order to eliminate impurity phases, different conditions including washing with water, different sintering temperatures, sintering times, and different atmospheres were studied. 

We washed the sample with water to eliminate impurity phases. It was observed that water-washing is somewhat effective for the elimination of the CaO and La2O3 impurity phases as indicated in Fig. 13(a). We can still see the Ca2Fe2O5 phase even after water-washing. It is observed that washing only with water is somewhat effective.

The sintering temperatures have been tested from 1000 °C to 1400 °C. As can be seen in Fig. 13(b), the impurity decreases with increasing temperature to about 1300 °C. Also at higher temperatures (1400 °C) the impurities increase and the original phase structure of the material changes.

Fig. 13(c) shows the XRD patterns of L58CCF-1000 samples prepared at 1000 ◦C for 5, 10, and 20 h in air, respectively. Increasing the sintering time had little effect on the impurity phase and the impurities remained.

Considering that the main material of L58CCF-1000 has a defective stoichiometry, it seemed that by taking oxygen from the sample and re-injecting it, the impurity could be forced to be present in the preferred lattice positions. Therefore, a small sample was annealed in argon for 5 hours at 1000 °C. A combination of two phases was again observed in the XRD pattern. Its structure was slightly different from the structure of the main material (also a change in color was observed in the sample). Of course, the formed phases had much higher peak intensities, more replaced peaks, and moved to lower angles. Therefore, the decision was made to anneal the sample again at temperatures of 900, 950, and 1000 °C in the air. The previous impurities appeared again, but it seems that they have both adjusted and that the main phase has become more pure. Baking in argon atmosphere and then in the air has rearranged the impurities. However, this method may be more useful in samples with partial impurities or for further purification of the main phase as well as the corresponding impurities. Fig. 2d shows the X-ray diffraction patterns of the L58CCF-1000 sintered in air, and argon.

\begin{figure}[!ht]
	\begin{center}
		\includegraphics[width=9cm,angle=0]{fig13}
		\vspace*{-0.4cm}
		\caption{ XRD patterns of the L58CCF composites synthesized at 1000 ◦C (a) after water-washing, (b) sintered at different temperatures, (c) for various sintering time, and (d) sintered in different atmospheres.  
			\label{fig13}}
	\end{center}
\end{figure}

According to the results, it seems that using higher temperatures for annealing of L58CCF-1000 is a more effective solution. Therefore, the prepared powders were annealed at 1300 °C for 5 h.


 Also, the results for the impurity amounts of L58SCF-1080 are shown in Fig. 14.(It is worth mentioning that due to the small amount of impurity, it was not possible to measure with maud, that is why the sum of the intensity of the impurity peaks and also the sum of the intensity of all the peaks were calculated and then the initial value was divided by the second value.)
 \begin{figure}[!ht]
 	\begin{center}
 		\includegraphics[width=8cm,angle=0]{fig14}
 		\vspace*{-0.4cm}
 		\caption{ Impurity percentage for  LSCF58-1080 tested in air from 25 to 1200 °C with consecutive heating/ cooling cycles.  
 			\label{fig14}}
 	\end{center}
 \end{figure}

\subsection{Reactivity and stability of  La$_{0.58}$M$_{0.4}$Co$_{0.2}$Fe$_{0.8}$$O_{3-\delta}$ (M = Sr or Ca) near the YSZ and GDC composite}

Fig.\ref{fig15}(a) and \ref{fig15}(b) shows the X-ray diffraction patterns of (La$_{0.58}$M$_{0.4}$Fe$_{0.8}$Co$_{0.2}$O$_{3-\delta}$) (M = Sr or Ca) and YSZ (50:50 wt\%) mixture sintered at 1080 ℃ for 0 h, 3 h and 20 h in air. For all composites, XRD data indicated a small peak shift to the left for the (La$_{0.58}$M$_{0.4}$Fe$_{0.8}$Co$_{0.2}$O$_{3-\delta}$) (M = Sr or Ca) peaks of the sintered samples as compared to the calcined powders. No shift is observed for YSZ peaks, so (La$_{0.58}$M$_{0.4}$Fe$_{0.8}$Co$_{0.2}$O$_{3-\delta}$) (M = Sr or Ca) shift is not a systematic error, but peak shifts are probably due to an increase in cell volume, which probably describes the solid state diffusion at partially melted boundaries between (La$_{0.58}$M$_{0.4}$Fe$_{0.8}$Co$_{0.2}$O$_{3-\delta}$) (M = Sr or Ca) and YSZ phases caused by diffusion of Zr4+ into the perovskite cation sublattice. Fig. 6(a) shows XRD analysis of the L58CFC-YSZ mixture powder shows that L58CFC reacts with YSZ and impurity phases CaZrO3 and CoFe2O4 spinel are formed. Also, no other phase like La2Zr2O7 was detected.La2Zr2O7 impurities were also observed for the L58SFC-YSZ (50:50 wt\%) mixture powder sintered for 20 h (Fig.\ref{fig15}(b)). For L58CFC and L58SFC, prepared samples, lattice parameters of the phases presented and Percentage of reaction between La$_{0.58}$M$_{0.4}$Fe$_{0.8}$Co$_{0.2}$O$_{3-\delta}$ (M = Sr or Ca) and YSZ are extracted from XRD data were listed in Table \ref{tab6}. The results show that the amount of undesired reaction with the YSZ for the L58CFC perovskites is less than the L58SFC perovskites.

 \begin{figure}[!ht]
	\begin{center}
			\includegraphics[width=9cm,angle=0]{fig15}
		\vspace*{-0.7cm}
		\caption{XRD patterns for mixture of (a) L58CCF and  YSZ (50:50), (b) L58SCF and YSZ (50:50) , and mixture of (c) L58CCF and 20GDC (50-50 wt\%), (d) L58SCF and 20GDC (50-50 wt\%) sintered at 1080 $^{\circ}$C for 0 h, 3 h and 20 h in air. 
			\label{fig15}}
	\end{center}
\end{figure}

\begin{table*}[h]
	\begin{center}
		\caption{Summary of lattice parameters extracted and impurity percentage from XRD data of the mixture of L58MCF (M=Sr and Ca) and YSZ with a weight ratio of 50:50 sintered at 1080 $^{\circ}$C for 0h, 3h and 20h.}
		\label{tab3}
		\begin{tabular}{|>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{1cm}|>{\centering\arraybackslash}m{1cm}|>{\centering\arraybackslash}m{1cm}|>{\centering\arraybackslash}m{1.1cm}|>{\centering\arraybackslash}m{1.1cm}|>{\centering\arraybackslash}m{1.7cm}|>{\centering\arraybackslash}m{0.9cm}|>{\centering\arraybackslash}m{0.9cm}|>{\centering\arraybackslash}m{0.9cm}|>{\centering\arraybackslash}m{1.1cm}|>{\centering\arraybackslash}m{1.05cm}|>{\centering\arraybackslash}m{1.05cm}|}
			\hline
			{Sample} & LCCF \textit{(Ortho.) a, b, c}& YSZ \textit{(Tet.) a=b, c}& CaZrO$ _{3} $ \textit{(Ortho.) a, b, c}& CoFe$ _{2} $O$ _{4} $ \textit{(Cub.)  a=b=c}& Impurity (\%)&{Sample}&L58SCF \textit{(Rhom.) a=b, c}&YSZ \textit{(Tet.) a=b, c}&SrZrO$ _{3} $ \textit{(Cub.) a=b=c}&CoFe$ _{2} $O$ _{4} $ \textit{(Cub.) a=b=c}&La$ _{2} $Fe$ _{2} $O$ _{7} $ \textit{(Cub.)}&Impurity (\%) \\	\hline
			L58CCF-YSZ (50:50wt.\%-0h)&5.4997 5.4806 7.7766&3.6374 5.1444& - & - &  - &L58SCF-YSZ (50:50wt.\%-0h)&5.4950 13.4750&3.6374 5.1444& - & - &  - & - \\ \hline
			L58CCF-YSZ (50:50wt.\%-3h)&5.5397 5.5853 7.8233&3.6427 5.1585&5.5860 7.9551 5.6868&8.3779&13&L58SCF-YSZ (50:50wt.\%-3h)&5.5976 13.7107&3.6458 5.1544&4.0600&8.3641&10.8076&25.96  \\ \hline
			L58CCF-YSZ (50:50wt.\%-20h)&5.6292 5.5778 7.8875&3.6556 5.1540&5.5998 8.1354 5.7646&8.3724&15.9&L58SCF-YSZ (50:50wt.\%-20h)&5.5980 13.7092&3.6468 5.1516&4.0600&8.3641&10.8076&26  \\ \hline
		\end{tabular}	
	\end{center}
\end{table*}

The chemical compatibility with GDC electrolytes was investigated by heating La$_{0.58}$M$_{0.4}$Fe$_{0.8}$Co$_{0.2}$O$_{3-\delta}$ (M = Sr or Ca)-20GDC (50:50 wt\%) composites at 1080 $^{\circ}$C for 0h, 3h and 20h is shown in Fig.\ref{fig15}. In all cases, the La$_{0.58}$M$_{0.4}$Fe$_{0.8}$Co$_{0.2}$O$_{3-\delta}$ (M = Sr or Ca) and the used electrolytes (20GDC) maintain their crystalline structures without any degradation. Every peak in the pattern can be attributed to either GDC or La0.58M0.4Fe0.8Co0.2O3-$\delta$ (M = Sr or Ca) and no impurity phases are observed, indicating great chemical compatibility between electrolyte (20GDC) and La$_{0.58}$M$_{0.4}$Fe$_{0.8}$Co$_{0.2}$O$_{3-\delta}$ (M = Sr or Ca).


